DFR-Net: Density Feature Refinement Network for Image Dehazing Utilizing Haze Density Difference

In image dehazing task, haze density is a key feature and affects the performance of dehazing methods. However, some of the existing methods lack a comparative image to measure densities, and others create intermediate results but lack the exploitation of their density differences, which can facilitate perception of density. To address these deficiencies, we propose a density-aware dehazing method named Density Feature Refinement Network (DFR-Net) that extracts haze density features from density differences and leverages density differences to refine density features. In DFR-Net, we first generate a proposal image that has lower overall density than the hazy input, bringing in global density differences. Additionally, the dehazing residual of the proposal image reflects the level of dehazing performance and provides local density differences that indicate localized hard dehazing or high density areas. Subsequently, we introduce a Global Branch (GB) and a Local Branch (LB) to achieve density-awareness. In GB, we use Siamese networks for feature extraction of hazy inputs and proposal images, and we propose a Global Density Feature Refinement (GDFR) module that can refine features by pushing features with different global densities further away. In LB, we explore local density features from the dehazing residuals between hazy inputs and proposal images and introduce an Intermediate Dehazing Residual Feedforward (IDRF) module to update local features and pull them closer to clear image features. Sufficient experiments demonstrate that the proposed method achieves results beyond the state-of-the-art methods on various datasets.

==> sections/6_conclusion.tex <==
\section{Conclusion}

This paper introduces various improvements for Swin Transformer applied to image dehazing, and the proposed DehazeFormer achieves superior performance on several datasets.
To summarize, we propose to use RescaleNorm and ReLU to replace the commonly used LayerNorm and GELU to avoid some negative effects that are not important for high-level vision tasks but critical for low-level vision tasks.
To improve the capability of MHSA, we propose a shifted window partitioning scheme based on reflection padding and a spatial information aggregation scheme using convolution in parallel with attention. 
We also propose some minor improvements that are applicable to other networks.
Finally, we collect a large-scale remote sensing image dehazing dataset to evaluate the network's capability to remove highly non-homogeneous haze, and DehazeFormer also achieves an impressive performance.
In the future, we plan to work on more lightweight and more straightforward architectures and extend the architecture to other low-level vision tasks. 
Besides, encoding feature maps on thumbnails and then decoding them on the original image may achieve real-time 4K image dehazing.

